Pricing Social Goods

Social goods are goods that grant value not only to their owners but also to the owners' surroundings, be it their families, friends or office mates. The benefit a non-owner derives from the good is affected by many factors, including the type of the good, its availability, and the social status of the non-owner. Depending on the magnitude of the benefit and on the price of the good, a potential buyer might stay away from purchasing the good, hoping to free ride on others' purchases. A revenue-maximizing seller who sells social goods must take these considerations into account when setting prices for the good. The literature on optimal pricing has advanced considerably over the last decade, but little is known about optimal pricing schemes for selling social goods. In this paper, we conduct a systematic study of revenue-maximizing pricing schemes for social goods: we introduce a Bayesian model for this scenario, and devise nearly-optimal pricing schemes for various types of externalities, both for simultaneous sales and for sequential sales.

==> app_grad.tex <==
Let $\p=(p_1,\ldots,p_n)$ be a price matrix posted by the seller, where $p_i=(p_i^0,\ldots, p_i^{i-1})$ is the price vector posted to agent $i$.
For every agent $i$, we define a set of thresholds $T_i^0,\ldots, T_i^{i-1}$, where $T_i^j(\p)$ is the minimal value for which agent $i$ buys the good \textit{conditioned} on $j$ agents buying the good prior to agent $i$ given the price matrix $\p$. We use the following notations:
\begin{enumerate}
	\item $q_{i,j}(\p)$: the probability that $j$ agents buy the good prior to the arrival of agent $i$, given prices $\p$.
	\item $r_{i,j}^k(\p)$: the probability that \textbf{exactly} $k$ agents buy a good given prices $\p$ and given that $j$ agents bought a good prior to agent $i$'s arrival. For ease of notations, we define $r_{n+1,j}^j=1$ and $r_{n+1,j}^k=0 $ for every $j \neq k$.
	\item $r_{i,j}^{< k}(\p) = \sum_{\ell=j}^{k-1}r_{i,j}^{\ell}$: the probability that \textbf{strictly less} than $k$ agents buy a good overall given prices $\p$ and given that $j$ agents bought a good prior to $i$'s arrival. 
\end{enumerate}
When clear from the context, we omit $\p$ and simply write $T_i^j, q_{i,j}, r_{i,j}^k$ and $r_{i,j}^{< k}$. Given these notations, we now describe the equilibrium condition for agent $i$. If agent $i$ does not buy a good when $j$ agents buy a good prior to her arrival, her utility from buying a good at price $p_i^j$ is $v_i-p_i^j$. On the other hand, if the agent does not buy a good, her expected utility is $v_i\cdot \sum_{\ell\geq j} w_\ell\cdot r_{i+1,j}^\ell$. Therefore, the threshold from which it is better for agent $i$ to buy an item when $j$ agents bought an item prior to agent $i$ satisfies:
\begin{eqnarray*}
	T_i^j-p_i^j=T_i^j\cdot \sum_{\ell\geq j} w_\ell\cdot r_{i+1,j}^\ell \Rightarrow p_i^j= T_i^j(1-\sum_{\ell\geq j} w_\ell\cdot r_{i+1,j}^\ell )
\end{eqnarray*}
Clearly, if $j$ agents bought the good prior to agent $i$'s arrival, then for every $\ell<j$, $r_{i+1,j}^\ell =0$. Therefore, we can rewrite the above condition as follows: 
\begin{eqnarray}
	p_i^j & = & T_i^j(1-\sum_{\ell\geq j} w_\ell\cdot r_{i+1,j}^\ell )\nonumber\\
	& = &T_i^j(w_n\cdot\sum_{\ell\geq j} r_{i+1,j}^{\ell}-\sum_{\ell\geq j} w_{\ell}\cdot r_{i+1,j}^\ell )\nonumber\\
%	& = & T_i^j\cdot\sum_{k=0}^n r_{i,j}^k(1- w_k)\nonumber\\
	& = & T_i^j\cdot\sum_{\ell\geq j} r_{i+1,j}^{\ell}(w_n- w_\ell)\nonumber\\
	& = & T_i^j\cdot\sum_{\ell\geq j} r_{i+1,j}^\ell \cdot\sum_{k>\ell}(w_{k}-w_{k-1})\nonumber\\
	& = & T_i^j\cdot\sum_{k>j}(w_{k}-w_{k-1})\cdot\sum_{\ell=0}^{k-1} r_{i+1,j}^\ell \nonumber\\
	& = & T_i^j\cdot\sum_{k>j}(w_{k}-w_{k-1})\cdot r_{i+1,j}^{< k},\label{eq:gradual_seq_eq}
\end{eqnarray}
where the second equality stems from $w_n=1$ and $\sum_{\ell\geq j} r_{i+1,j}^\ell =1$.

Notice that for $j\geq i$, $q_{i,j}=0$.
 We therefore can express the revenue from setting prices $\p$ as:
\begin{eqnarray}
	\rev(\p)& = &\sum_{i,j} q_{i,j} \cdot p_i^j\cdot(1-F_i(T_i^j))\nonumber\\
	& = & \sum_{i,j} q_{i,j}\cdot T_i^j\cdot \sum_{k>j}(w_{k}-w_{k-1})\cdot r_{i+1,j}^{<k}\cdot(1-F_i(T_i^j))\nonumber\\
	& = & \sum_{k=1}^{n}(w_{k}-w_{k-1})\cdot \sum_{i}\sum_{j< k} q_{i,j}\cdot T_i^j\cdot (1-F_i(T_i^j))\cdot r_{i+1,j}^{< k}.\label{eq:grad_seq_eq_rev}
\end{eqnarray}

For a given vector of thresholds $\TT$ and a given $k$, let $$\revpubseqmult(\TT)=\sum_{i}\sum_{j<k} q_{i,j}\cdot T_i^j\cdot (1-F_i(T_i^j))\cdot r_{i+1,j}^{< k}.$$
As defined is Section \ref{section:posted_prices}, let $\RR(\F,\mathcal{J}_k,\sigma,\p)$ be the revenue of a posted price mechanism for agents drawn from a product distribution $\F$, and offered prices $\p$ sequentially, according to order $\sigma$, until $k$ items are sold. Since we assume that agents arrive according to their index, we omit $\sigma$ from now on. We denote by $\RR^*(\F,\mathcal{J}_k)$ the revenue of the optimal posted price mechanism for selling $k$ private items sequentially in the same order of arrival as in our social goods setting.  
We have the following:
\BL
For every threshold vector $\TT$ and every number of items $k$, 
\begin{eqnarray*}
	\revpubseqmult(\TT)\leq \RR^*(\F,\mathcal{J}_k). \label{lm:revpubmultbound}
\end{eqnarray*}
\EL
\BPF
We assume by renaming that the agents arrive in the order of their index. Let us define the following posted prices sale for selling $k$ items privately. We define the price matrix $\hat{\p}$, where 
$${\hat{p}}_i^j=\begin{cases} T_i^j\quad & j< k\\ \infty\quad & \mbox{otherwise}\end{cases}.$$ 
When agent $i$ arrives, the seller posts a price of ${\hat{p}}_i^j$ if $j$ goods where purchased prior to agent $i$'s arrival.

For $j< k$, let  $\hat{q}_{i,j}$ be the probability that $j$ items are sold prior to the arrival of agent $i$. We show by induction on $i$ that for every $i$ and $j$ $\hat{q}_{i,j}=q_{i,j}$. For the first agent to arrive (\textit{i.e.}, $i=1$), clearly $q_{i,0}=\hat{q}_{i,0}=1$ (and obviously, $q_{i,j}=\hat{q}_{i,j}=0$ for every other $j$). Let us assume that the claim holds for agent $i$ (and for every $j$). It is clear that for $j< k$, $$q_{i+1,j}=q_{i,j-1}\cdot (1-F_{i}(T_{i}^{j-1}))+q_{i,j}\cdot F_i(T_i^j)={\hat{q}}_{i,j-1}\cdot (1-F_{i}({\hat{p}}_{i}^{j-1}))+{\hat{q}}_{i,j}\cdot F_i({\hat{p}}_i^j)={\hat{q}}_{i+1,j}.$$


Therefore, the revenue from selling $k$ items in a private sale using prices $\hat{\p}$ can be expressed by:
\begin{eqnarray*}
	\sum_{i}\sum_{j< k} {\hat{q}}_{i,j} \cdot {\hat{p}}_i^j \cdot (1-F_i({\hat{p}}_i^j)) & = &  \sum_{i}\sum_{j<k} {q}_{i,j} \cdot {T}_i^j \cdot (1-F_i({T}_i^j))\\
	&\geq & \sum_{i}\sum_{j<k} q_{i,j}\cdot T_i^j\cdot (1-F_i(T_i^j))\cdot r_{i+1,j}^{< k}\\
	& = & \revpubseqmult(\TT).
\end{eqnarray*}
Since selling $k$ items using prices $\hat{\p}$ is a private posted price sale of at most $k$ items, the revenue obtained by this sale is at most that of the optimal posted price sale for selling $k$ items, $\RR^*(\F,\mathcal{J}_k)$. Therefore, we get the desired result.
\EPF

	For $k>n$, we set $w_k=1$. Using Lemma \ref{lm:revpubmultbound}, we can bound inequality $(\ref{eq:grad_seq_eq_rev})$ and get:

\begin{eqnarray*}
\rev(\p)& \leq& \sum_{k=1}^{n}(w_{k}-w_{k-1})\cdot \RR^*(\F,\mathcal{J}_k)\\
&= &\sum_{\ell=0}^{\lfloor\log n\rfloor}\sum_{k=2^\ell}^{2^{\ell+1}-1}(w_{k}-w_{k-1})\cdot \RR^*(\F,\mathcal{J}_k)\\
& \leq & \sum_{\ell=0}^{\lfloor\log n\rfloor}\sum_{k=2^\ell}^{2^{\ell+1}-1}(w_{k}-w_{k-1})\cdot \RR^*\left(\F,\mathcal{J}_{\min(2^{\ell+1}-1,n)}\right)\\
& = & \sum_{\ell=0}^{\lfloor\log n\rfloor}(w_{2^{\ell+1}-1}-w_{2^{\ell}-1})\cdot \RR^*\left(\F,\mathcal{J}_{\min(2^{\ell+1}-1,n)}\right),
\end{eqnarray*}
where the second equality stems from $(w_{k}-w_{k-1})\cdot \RR^*(\F,\mathcal{J}_k)=(1-1)\cdot \RR^*(\F,\mathcal{J}_k)=0$ for $k>n$. 

In order to show an $O(\log n )$ approximation to the optimal sequential posted price sell, we show how to produce a sale of revenue $\Omega(1)\cdot (w_{2k+1}-w_{k})\cdot \RR^*(\F,\mathcal{J}_{2k+1})$ for every $k\leq n $. 

\BL
	For every $k\in \{1,\ldots,n\}$, there exist prices $\p$ that guarantee an expected revenue of $\Omega(1)\cdot (w_{2k+1}-w_{k})\cdot \RR^*(\F,\mathcal{J}_{2k+1})$.\label{lem:grad1}
\EL
\BPF
	As described in Section \ref{section:posted_prices}, let $\hat{\p}$ be a set of near optimal posted prices used by an OPM, which can be found according to Theorem \ref{thm:k_uniform_rev}. We define the prices of our sequential public model in a way that ensures that for every agent $i$ and for every $j< k$, $T_i^j=\hat{p}_i$ (and $T_i^j=\infty$ for $j\geq k$). 
	This can be done using the following:
	\begin{itemize}
		\item For agent $n$, set $p_n^j=\hat{p}_n\cdot\left(1-w_j\right)$ for every $j< k$, and $p_n^j=\infty$  for $j\geq k$. Set $r_{n,j}^j=F_n(T_n^j)$, $r_{n,j}^{j+1}=1-F_n(T_n^j)$. Notice this enforces the thresholds we described above, and the $r_{n,j}^k$'s are matching our definitions.
		\item For agent $i<n$, given $r_{i+1,j}^k$ for every $j$ and $k$, we set $p_i^j= \hat{p}_i (1-\sum_{\ell\geq j} w_\ell\cdot r_{i+1,j}^\ell )$ for every $j< k$, and $p_i^j=\infty$ for $j\geq k$. Set $$r_{i,j}^k=F_i(T_i^j)\cdot r_{i+1,j}^k +(1-F_i(T_i^j))\cdot r_{i+1,j+1}^k.$$ Given the $r_{i+1,j}^k$'s are computed correctly, this enforces the thresholds we described above, and the  $r_{i,j}^k$'s also match the computed thresholds.
	\end{itemize}
	Notice that for every $i$ and  $j<\min(i,k)$, we have that:
	\begin{eqnarray}
		p_i^j & = & \hat{p}_i \left(1-\sum_{\ell\geq j} w_\ell\cdot r_{i+1,j}^\ell\right) \nonumber \\
		& \geq & \hat{p}_i \left(1-\sum_{\ell= j}^{k} w_k\cdot r_{i+1,j}^\ell - \sum_{\ell= k+1}^{n} w_\ell \cdot r_{i+1,j}^\ell\right) \nonumber\\
		& = & \hat{p}_i \left(1-w_k\sum_{\ell= j}^{k}  r_{i+1,j}^\ell\right)\nonumber\\
		& = &  \hat{p}_i (1-w_k),\label{eq:price_grad_lb}
	\end{eqnarray}
	where the second equality stems from the fact that after selling $k$ items, all prices are set to $\infty$, which implies that $r_{i+1,j}^\ell=0$, and the last equality is because $\sum_{\ell= j}^{k}  r_{i+1,j}^\ell=1$.
	
	Let $q_{i}^{< k}$ denote the probability that less than $k$ items  were sold prior to the arrival of agent $i$. Setting the thresholds and prices as described above, we get that the expected revenue is:
	\begin{eqnarray}
		\sum_{i,j} q_{i,j}\cdot p_i^j\cdot (1-F_i(T_i^j)) & = & \sum_{i}\sum_{j=0}^{\min(i-1,k-1)} q_{i,j}\cdot p_i^j\cdot (1-F_i(\hat{p}_i))\nonumber\\
		&\geq & \sum_{i}\sum_{j=0}^{\min(i-1,k-1)} q_{i,j}\cdot \hat{p}_i (1-w_k)\cdot (1-F_i(\hat{p}_i))\nonumber\\
		& = & (1-w_k)\sum_{i}q_{i}^{< k} \cdot \hat{p}_i\cdot (1-F_i(\hat{p}_i))\nonumber\\
		& \geq & (w_{2k+1}-w_k)\sum_{i}q_{i}^{< k} \cdot \hat{p}_i\cdot (1-F_i(\hat{p}_i))\nonumber\\
		& \geq & (w_{2k+1}-w_k)\cdot \Omega(1)\cdot \RR^*(\F,\mathcal{J}_{k})\nonumber\\
		& \geq &  \Omega(1)\cdot (w_{2k+1}-w_k)\cdot\RR^*(\F,\mathcal{J}_{2k+1}),\label{eq:grad_log}
	\end{eqnarray}
	where the first equality stems from the fact that we set $T_i^j=\hat{p}_i$ for $j<k$, the first inequality is due to (\ref{eq:price_grad_lb}), and the third inequality is because $q_{i}^{< k}$ is exactly the probability that agent $i$ is approached in the posted price sale with no externalities when using $\hat{\p}$ as prices. 
	
\EPF

\BL
  There exist prices $\p$ that guarantee an expected revenue of $\Omega(1)\cdot \RR^*(\F,\mathcal{J}_{1})$.\label{lem:grad2}
\EL
\BPF
	Let $\hat{\TT}$ be a set of thresholds which approximate $\rbestseq(\F)$ in the fully public good model, and let $\hat{\p}=\tr^{-1}(\hat{\TT})$  be the prices for which $\hat{\TT}$ is the equilibrium in that model. By Theorem \ref{thm:canonical-rev}, the revenue achieved using these prices is $\Theta(1)\cdot \RR^*(\F,\mathcal{J}_{1})$; \textit{I.e.},
	\begin{eqnarray}
		\sum_i \left(\prod_{j<i}F_j(\hat{T}_j)\right)\cdot \hat{p}_i\cdot(1-F_i(\hat{T}_i))= \Theta(1)\cdot \RR^*(\F,\mathcal{J}_{1}).\label{eq:fully_rev_bound}
	\end{eqnarray} 
	
	In the model with gradually increasing externalities, we set prices $\p$ such that for every agent $i$, $T_i^0=\hat{T}_i$ and $T_i^j=\infty$ for every $j>0$; \textit{I.e.}, sell to the agent with probability $F_i(\hat{T}_i)$ \textbf{only if} no agent purchased a good prior to the arrival of the agent. These thresholds can be computed using the following:
	\begin{itemize}
		\item For agent $n$, set $p_n^0=\hat{T}_n$ and $p_n^j=\infty$ for $j>0$. 
		\item For agent $i<n$, set: 
		\begin{eqnarray}
			p_i^0  =  \hat{T}_i\cdot(1-\sum_{\ell\geq 0}w_{\ell}\cdot r_{i+1,0}^{\ell})
			 =  \hat{T}_i\cdot(1-w_{1}\cdot r_{i+1,0}^{1})
			 =  \hat{T}_i\cdot\left(1-w_{1}\cdot \left(1-\prod_{j>i}F_j(\hat{T}_j)\right)\right),\label{eq:threshold_prices_grad}
		\end{eqnarray}
		and $p_i^j=\infty$ for $j>0$.
		%We note that by setting the thresholds as described above, we have that $r_{i+1,0}^1=\left(1- \prod_{j>1}F_j(T_j) \right)$ for 
	\end{itemize}
	Note that by (\ref{eq:threshold_prices_grad}), we have that $$p_i^0= \hat{T}_i\cdot\left(1-w_{1}\cdot \left(1-\prod_{j>i}F_j(\hat{T}_j)\right)\right)\geq \hat{T}_i\cdot(1- (1-\prod_{j>i}F_j(\hat{T}_j)))=\hat{T}_i\cdot\prod_{j>i}F_j(\hat{T}_j)=\hat{p}_i,$$ where the last equality is due to the equilibrium condition of the fully public sequential model (\ref{eq:eq_condition_seq}).
	
	We get that the revenue in the model with gradually increasing externalities is:
	\begin{eqnarray*}
		\sum_{i,j}q_{i,j}\cdot p_i^j\cdot(1-F_i(T_i^j)) & = & \sum_{i}q_{i,0} \cdot p_i^0\cdot (1-F_i(T_i^0))\\
		& \geq & \sum_{i}\left(\prod_{j<i}F_j(T_j^0)\right) \hat{p}_i(1-F_i(\hat{T}_i))\\
		& = & \sum_{i}\left(\prod_{j<i}F_j(\hat{T}_j)\right) \hat{p}_i(1-F_i(\hat{T}_i))\\
		& = & \Theta(1)\cdot \RR^*(\F,\mathcal{J}_{1}).
	\end{eqnarray*}
	
	
\EPF

By combining Equation $(\ref{eq:grad_log})$ with Lemmata \ref{lem:grad1} and \ref{lem:grad2} the proof of Theorem \ref{thm:grad_main} is completed.

==> fullproofs.tex <==

%As a consequence of (ii), $\rbwseq(\F) = \Theta(1)\cdot \rbestseq(\F)$.
\EC
%\BPF
%	Follows directly from Theorems \ref{thm:homog_prices} and \ref{thm:anonymous_e}.
%\EPF

%\subsubsection{Implications to public goods}
%TBD (pending reading the FOCS 2015 paper) 

==> general-graphs.tex <==



==> hard_seq.tex <==
Let $k$ be the size of the maximum independent set in $G$. By fixing a maximum size independent set, and offering a price of $1/2$ to each agent $i$ in the set, we get a revenue of $1/2$ from agent $i$ (and a price $>1$ for all other agents). This is true since none of agent $i$'s neighbors purchase a good. Therefore, we get that $\rbestseq(\F)\geq k/2$. Since we assume tie-breaking is done consistently, we can assume that $v_i\neq p_i$ for every $i$.
We now show how to compute an equilibrium:
\\\\
\MyFrame{	
	\begin{enumerate}
		\item[] $S \gets \emptyset$
		\item[] For $i=n,\ldots,1$:
		\begin{itemize}
			\item[] If $(p_i< v_i)$ and $N(i) \cap S =\emptyset$:
			\begin{itemize}
				\item[] $S=S \cup \{i\}$
			\end{itemize}		
		\end{itemize}
	\end{enumerate}
}
\\\\
We claim that in a subgame perfect equilibrium, only agents in $S$ buy a good. We show it by induction on the number of agents. For $n=1$, this is trivial, since the single agent buys if and only if $p_i<v_i$. Let us assume the claim is true for $n<n'$, and show the claim for $n=n'$. Let us inspect the first agent to arrive. We inspect two cases:
\begin{enumerate}
	\item The first agent does not buy a good (\textit{i.e.}, the first agent is not in $S$): this implies one of the following. 
	\begin{itemize}
		\item $v_1<p_1$. In this case the agent has a negative utility of purchasing the good and he would not buy. 
		\item  A neighboring agent purchases a good and the first agent has a utility of $v_1$, which is greater than $v_1-p_1$, the utility of the agent if she were to purchase a good. After the first agent does not buy a good, this is equivalent to a network without the first agent, and by the inductive assumption, the rest of the players are in a subgame perfect equilibrium. This is, one of the neighbors of the first agent buys a good. Therefore, the first agent gets a higher utility in the subgame perfect equilibrium induced by the agent not buying a good.
	\end{itemize} 
	We get that in this case, the first agent does not buy in an equilibrium. Since this is equivalent to a network without the first agent, by the inductive assumption, the rest of the players are in a subgame perfect equilibrium when set $S$ is the purchasing set.
	
	\item The first agent buys a good (the first agent is in $S$). This implies that $v_1>p_1$ and that non of the agent's neighbors is in $S$ ($N(1)\cap S=\emptyset$). Therefore, if the first agent buys a good, her utility is $v_1-p_1>0$.
	If the first agent were not to buy a good, this would have been equivalent to a network without the first agent. By the inductive assumption, in an equilibrium, the set $S-\{1\}$ would  have bought a good. Therefore, non of agent 1's neighbors would have bought a good, and her utility would have been $0$. This implies that in equilibrium, the first agent buys.
	
	Whenever the first agent buys a good, her neighbors do not buy a good, and this is equivalent to a network without the first agent and the agents in $N(1)$. It is not hard to verify that in this case, the computation above returns the set $S-\{1\}$ as a purchasing set. This follows since the non-purchasing agents have no effect on the agents that arrive prior to them or after them in the computation. That is, the set $S$ buys overall in the equilibrium where the first agent buys. 
\end{enumerate}
We get that in both cases, the subgame perfect equilibrium is for agents in set $S$ to purchase a good, which completes the inductive proof.

Notice that in the equilibrium computed above, the set $S$ of purchasing agents is an independent set, and therefore, $\sum_{i\in S} p_i\leq \abs{S}\leq k$. Our reduction from maximum independent set computes $S$ and returns $\abs{MAX-IS} = \sum_{i\in S} p_i$. We conclude that if the algorithm finds prices such that $\rseq(\F, \p)\geq \frac{\rbestseq(\F)}{O(n^{1-\epsilon})}$, we can compute a number in $\left[\frac{k}{O(n^{1-\epsilon})},k\right]$, which is $\mathrm{NP}$-hard according to Theorem \ref{thm:max-is-nphard}.


==> semi_sim.tex <==
	Recall that $\p=(p_1,\ldots, p_n)$ is the price vector posted by the seller, where $p_i$ is the price offered to agent $i$, and let $\TT$ be some equilibrium induced by $\p$ (therefore, $\TT$ satisfies Equation $(\ref{eq:equilibrium_fading_sim})$).
		The revenue of the sale when $\p$ are the prices and $\TT$ is equilibrium can be expressed by: 
		\begin{eqnarray}
			\rev(\p,\TT) & = & \sum_i  p_i\cdot (1-F_i(T_i))\nonumber\\
			& = & \sum_i \left((1-w_i) \cdot T_i + w_i \cdot T_i \cdot \prod_{j\neq i}{F_j(T_j)}\right)\cdot (1-F_i(T_i)) \nonumber\\
			& = & \sum_i (1-w_i) \cdot T_i \cdot (1-F_i(T_i))+
			\sum_i w_i \cdot T_i \cdot \left(\prod_{j\neq i}{F_j(T_j)}\right) \cdot (1-F_i(T_i))\nonumber\\
			& \leq & \sum_i (1-w_i) \cdot T_i \cdot (1-F_i(T_i))+
			\sum_i T_i \cdot \left(\prod_{j\neq i}{F_j(T_j)}\right) \cdot (1-F_i(T_i))\nonumber\\
			& = & \rev_1(\TT,\w) + \rev_2(\TT)\nonumber\\
			& \leq & \max_{\hat{\TT}}\rev_1(\hat{\TT},\w)+ \max_{\hat{\TT}}\rev_2(\hat{\TT}). \label{eq:rev_bound_fade_sim}
		\end{eqnarray}
		
		We now show that it is possible to find prices that approximate $\max_{\hat{\TT}}\rev_1(\hat{\TT},\w)$ and prices that approximate $\max_{\hat{\TT}}\rev_2(\hat{\TT})$. This yields a constant approximation for our model.

		\BL
			One can compute prices $\p$ such that the expected revenue $\rmin(\p)\geq \max_{\TT}\rev_1(\TT,\w)$.\label{lm:rev_priv_sim}
		\EL
		\BPF
			Let $\hat{\p}$ be a vector such that $\hat{p}_i$ is the monopolist price for distribution $F_i$. Notice that $\hat{\p}=\argmax_{\TT}\rev_1(\TT,\w)$ for every $\w$.
			We set prices $\p$ such that for every $i$, $$p_i=(1-w_i)\cdot \hat{p}_i.$$
			
			We first show that in every equilibrium $\TT$,  $T_i\leq \hat{p}_i$. By Equation $(\ref{eq:equilibrium_fading_sim})$, we get: 
			$$T_i=\frac{p_i}{(1-w_i)+w_i\cdot\prod_{j\neq i} F_j(T_j)}\leq  \frac{(1-w_i)\cdot \hat{p}_i}{(1-w_i)}=\hat{p}_i.$$
			
			
			We get that for every $\TT$, the expected revenue from setting prices $\p$ is at least:
			\begin{eqnarray*}
				\rev(\p,\TT) & = & \sum_i p_i\cdot (1-F_i(T_i))\\
				& \geq & \sum_i (1-w_i)\cdot \hat{p}_i\cdot (1-F_i(\hat{p}_i))\\
				& = & \rev_1(\hat{\p},\w)\\
				& = &\max_{\TT}\rev_1(\TT,\w),
			\end{eqnarray*}
			as desired.	
		\EPF
		
		\BL
			One can compute prices $\p$ such that the expected revenue $\rev(\p)\geq \Omega(1)\cdot\max_{\TT}\rev_2(\TT)$.\label{lm:rev_pub_sim}
		\EL
		\BPF		
			Let $\hat{p}$ be an anonymous price for which
			\begin{eqnarray}
				\hat{p}\cdot\left(1-\prod_{i} F_i(\hat{p}_i)\right)=  \Omega(1)\cdot Myer(\F)= \Omega(1) \cdot \rev_2(\F).\label{eq:anonymous_fade_sim}
			\end{eqnarray}
			This uniform price exists according to \cite{DBLP:journals/corr/AlaeiHNPY15}.
			We post a uniform price vector $\p$ such $p_i=\hat{p}/2$ for every $i$. 
			Let $\RR=\hat{p}\cdot (1-\prod_i F_i(\hat{p}))$ be the revenue of an anonymous price mechanism which posts a price $p$. 
Given an equilibrium strategy vector $\TT$, we have that the expected revenue is at least $\frac{\hat{p}}{2}\cdot (1-\prod_i F_i(T_i))$, since more then one agent might purchase an item. 
\begin{enumerate}
	\item $T_i\leq \hat{p}$ for every agent $i$: In this case, since the CDFs are monotonically non-decreasing, we have that $\frac{\hat{p}}{2}\cdot (1-\prod_i F_i(T_i))\geq \frac{\hat{p}}{2}\cdot (1-\prod_i F_i(\hat{p}))=\RR/2$.
	\item There exists an agent $i$ such that $T_i> \hat{p}$: By the equilibrium condition $(\ref{eq:equilibrium_fading_sim})$, we have that $T_i=\frac{\hat{p}/2}{(1-w_i)+w_i\cdot \prod_{j\neq i} F_j(T_j)}>\hat{p}$. Which yields $(1-w_i)+w_i\cdot \prod_{j\neq i} F_j(T_j)< \frac{1}{2}$. We get:
	\begin{eqnarray*}
		\prod_{j} F_j(T_j) & \leq & \prod_{j\neq i} F_j(T_j)\\
		& =  &(1-w_i)\cdot  \prod_{j\neq i} F_j(T_j) + w_i\cdot \prod_{j\neq i} F_j(T_j)\\
		& \leq & (1-w_i)+ w_i\cdot \prod_{j\neq i} F_j(T_j)\\
		& < & \frac{1}{2}.
	\end{eqnarray*}
	That is, the expected revenue is at least: $$\frac{\hat{p}}{2}\cdot (1-\prod_i F_i(T_i))>\frac{\hat{p}}{4}= \Omega(1)\cdot Myer(\F)= \Omega(1)\cdot \rev_2(\F),$$ as desired.
\end{enumerate} 


		\EPF
		
The proof of Theorem \ref{thm:semi_sim_main} follows from Equation $(\ref{eq:rev_bound_fade_sim})$, and Lemmata \ref{lm:rev_priv_sim} and \ref{lm:rev_pub_sim}.


==> vegtables.tex <==
	\textbf{Remark:} This is only for the simultaneous model, should look into sequential. 
	\textbf{Remark:} Show that best EFP is a constant approximation from best EHP. 
	
	
	\textbf{FPE:} for Fixed Prices Equilibrium.
	\textbf{HPE:} Heterogeneous Prices Equilibrium.
	
	\begin{tabular}{|c|c|c|c|c|c|}
		\hline  & Worst FPE & Best FPE & Worst HPE & Best HPE & MAX IS Price \\ 
		\hline Worst FPE & 1 & $\Omega(n)$ [\ref{subsec:fixedbestvsworst}] & $\Omega(n)$ [\ref{subsec:heteroworstfixedvsworst}]&  &\\ 	
		\hline Best FPE &  & 1 &  & & \\ 
		\hline Worst HPE  &  &  & 1 &   &\\ 
		\hline Best HPE &  &  &  & 1 & \\ 
		\hline 
	\end{tabular} 
	
	\subsection{Example where best and worst fix prices differ by $\Omega{(n)}$}\label{subsec:fixedbestvsworst}
	Consider a graph $K_{n,n}$ and $F=U[0,1]$. The symmetric equilibrium for some fixed price $p$ for which $p=T\cdot T^{n}\Rightarrow T=\sqrt[n+1]{p}$ holds. In this case, the expected revenue is $2np(1-F(T))=nT^{n+1}(1-T)$. Using derivatives, we get that this is maximized for $T=(n+1)/(n+2)$, and the revenue for a symmetric equilibrium is at most $2(1-1/(n+2))^n\leq 2$.
	
	On the other hand, setting $p=1/2$, there exists an equilibrium for which $T_A=p$ and $T_B=1$. In this  equilibrium, the expected revenue is $n/4$. 
	
	\subsection{Example where worst heterogeneous equilibrium and worst fix price equilibrium differ by $\Omega{(n)}$}\label{subsec:heteroworstfixedvsworst}
	
	Setting $p_A=1/2$ and $p_B=1$ gives the same equilibrium as the last example from above.
	
	
	\subsection{Meeting summary 4/03/15}
	Questions arose:
	\begin{enumerate}
		\item Is the Myer/4 bound tight? Is there a better bound for the sequential case?
		\item What about the simultaneous case? Can we do anything?
		\item What about if the seller can only offer only a restricted number of offers?
		\item Two items single minded buyers. How does the equilibrium look like? Are there thresholds with a single transition points? Is there a way to get an optimal mechanism?
		\item What is the best posted price mechanism for a single items multiple buyers?
		
	\end{enumerate}
	
	\section{old works, not relevant}
	
	\subsection{Sequential vs. Simultaneous gap}
	
	Here we show that although setting prices such that $\phi_i(T_i)=t$ for every $i$ approximates the Myerson revenue in the sequential case, it does not necessarily approximate it in the simultaneous case, even in the case of two buyers. Let $F_1(v)= 1-(1-v)^k$ for some integer $k$ be the distribution of the first buyer, and let $F_2(v)=\left(\frac{v}{1+\epsilon}\right)^\ell$ be the distribution of the second one. It is easy to see that both distributions are regular (see figure TBD).  We set $T_1=1$ and $T_2=\frac{1+\epsilon}{\sqrt[\ell]{2}}$. Notice that $F_1(T_1)=1$ and $F_2(T_2)=1/2$. Let $\phi_1(v)=1/k+v\cdot\frac{k-1}{k}$ and $\phi_2(v)=v-\frac{(1+\epsilon)^\ell-v^\ell}{\ell v^{\ell-1}}$ be the virtual value functions of $F_1$ and $F_2$ respectively. Since $\phi_1(T_1)=\phi_1(1)=1$, we want that $\phi_2(T_2)=T_2-\frac{(1+\epsilon)^\ell-T_2^\ell}{\ell T_2^{\ell-1}}=1$. Solving this constraint yields that $\epsilon= \frac{\ell\sqrt[\ell]{2}}{\ell-1}-1$. 
	
	Applying the equilibrium conditions gives us $p_1=T_1\cdot F_2(T_2)=1/2$ and $p_2=T_2\cdot F_1(T_1)=T_2$. Let $T'_1=1/2$ and $T'_2=\frac{1+\epsilon}{\sqrt[\ell]{2}}\cdot\frac{2^k}{2^k-1}$. Since for every $v\geq 1+\epsilon$, $F_2(v)=1$, we want to choose $k$ and $\ell$ such that $\frac{2^k}{2^k-1}\geq\sqrt[\ell]{2}$. We get that $T'_1\cdot F_2(T'_2)=1/2=p_1$ and $T'_2\cdot F_1(T'_1)=\frac{1+\epsilon}{\sqrt[\ell]{2}}\cdot\frac{2^k}{2^k-1}\cdot\frac{2^k-1}{2^k}= \frac{1+\epsilon}{\sqrt[\ell]{2}}=T_2=p_2$. Therefore, $T'_1$ and $T'_2$ satisfy the equilibrium conditions. 
	
	The expected revenue out of the equilibrium thresholds $T_1$ and $T_2$ is $(1-F(T_2))p_2=T_2/2=\left(\frac{1+\epsilon}{\sqrt[\ell]{2}}\right)/2$. For a large enough $\ell$ we get that this tends to $1/2$. On the other hand the expected revenue out of the equilibrium thresholds $T'_1$ and $T'_2$ is $p_1\cdot (1-F_1(T'_1))=\left(\frac{1}{2^k}\right)/2$.


\section{Two items two agents}

\subsection{public equilibrium}
Prices - $p^a,p^b,p^{ab}$, $p'^a\ldots$.
Given thresholds of agent 2, $T'_1,\ldots,T'_4$, the following probabilities are defined:
\begin{itemize}
	\item $S'_1=(1-T'_1)T'_4$.	
	\item $S'_2=(1-T'_2)T'_3$.
	\item $S'_3=(1-T'_3)(1-T'_4)-\frac{(T'_1-T'_3)(T'_2-T'_4)}{2}$.
	\item $S'_0=T'_1 T'_2-\frac{(T'_1-T'_3)(T'_2-T'_4)}{2}$.
\end{itemize}
The probability of agent 2 buying item $a$ is $q'_a=S'_1+S'_3$, the probability of agent 2 buying item $b$ is $q'_b=S'_2+S'_3$.

\begin{enumerate}
	\item Value of 1 when not buying anything: $v_{a} q'_a +v_{b} q'_b$.\label{val0}
	\item Value of 1 when buying $a$: $v_{a}-p^a+v_{b} q'_b$.\label{vala}
	\item Value of 1 when buying $b$: $v_{b}-p^b+v_{a} q'_a$.\label{valb}
	\item Value of 1 when buying both: $v_{a}+v_b-p^{ab}$.\label{valboth}
\end{enumerate}

Best response of agent 1, given $T'_1,\ldots,T'_4$:
\begin{itemize}
	\item $\ref{val0}+\ref{vala}\Rightarrow T_1=\frac{p^a}{1-q'_a}$.
	\item $\ref{val0}+\ref{valb}\Rightarrow T_2=\frac{p^b}{1-q'_b}$.
	\item $\ref{vala}+\ref{valboth}\Rightarrow T_4=\frac{p^{ab}-p^a}{1-q'_b}$.
	\item $\ref{valb}+\ref{valboth}\Rightarrow T_3=\frac{p^{ab}-p^b}{1-q'_a}$.
\end{itemize}

TODO: show graph

TODO: show fixed point argument for equilibrium 

